SPINEPS -- Automatic Whole Spine Segmentation of T2-weighted MR images using a Two-Phase Approach to Multi-class Semantic and Instance Segmentation

Purpose. To present SPINEPS, an open-source deep learning approach for semantic and instance segmentation of 14 spinal structures (ten vertebra substructures, intervertebral discs, spinal cord, spinal canal, and sacrum) in whole body T2w MRI. Methods. During this HIPPA-compliant, retrospective study, we utilized the public SPIDER dataset (218 subjects, 63% female) and a subset of the German National Cohort (1423 subjects, mean age 53, 49% female) for training and evaluation. We combined CT and T2w segmentations to train models that segment 14 spinal structures in T2w sagittal scans both semantically and instance-wise. Performance evaluation metrics included Dice similarity coefficient, average symmetrical surface distance, panoptic quality, segmentation quality, and recognition quality. Statistical significance was assessed using the Wilcoxon signed-rank test. An in-house dataset was used to qualitatively evaluate out-of-distribution samples. Results. On the public dataset, our approach outperformed the baseline (instance-wise vertebra dice score 0.929 vs. 0.907, p-value<0.001). Training on auto-generated annotations and evaluating on manually corrected test data from the GNC yielded global dice scores of 0.900 for vertebrae, 0.960 for intervertebral discs, and 0.947 for the spinal canal. Incorporating the SPIDER dataset during training increased these scores to 0.920, 0.967, 0.958, respectively. Conclusions. The proposed segmentation approach offers robust segmentation of 14 spinal structures in T2w sagittal images, including the spinal cord, spinal canal, intervertebral discs, endplate, sacrum, and vertebrae. The approach yields both a semantic and instance mask as output, thus being easy to utilize. This marks the first publicly available algorithm for whole spine segmentation in sagittal T2w MR imaging.

==> flow/acronyms2.tex <==
\usepackage[nolist]{acronym}


\begin{acronym}
    \acro{AP}{Average Precision}
    \acro{ADC}{Apparent diffusion coefficient}
    \acro{ASSD}{Average Symmetric Surface Distance}
    \acro{AUC}{Area Under the Curve}
    \acro{BraTS-M}{ASNR-MICCAI BraTS Brain Metastasis Challenge}
    \acro{BraTS-G}{RSNA-ASNR-MICCAI BraTS Continuous Evaluation Challenge}
    \acro{CNN}{Convolutional Neural Network}
    \acro{CCA}{Connected Component Analysis}
    \acro{CT}{Computed Tomography}
    \acro{clDice}{Centerline Dice Similarity Coefficient}
    \acro{DL}{Deep Learning}
    \acro{DQ}{Detection Quality}
    \acro{TP}{True Positive}
    \acro{FP}{False Positive}
    \acro{FN}{False Negatives}
    \acro{DSC}{Dice Similarity Coefficient}
    \acro{DWI}{Diffusion Weighted Imaging}
    \acro{ET}{Enhancing Tumor}
    \acro{GAN}{Generative Adversarial Network}
    \acro{gvDSC}{global volumetric Dice Similarity Coefficient}
    \acro{HD}{Hausdorff Distance}
    \acro{ISLES}{Ischemic Stroke Lesion Segmentation 2022 challenge}
    \acro{IOU}{Intersection over Union}
    \acro{InS}{Instance Segmentation}
    \acro{ML}{Machine Learning}
    \acro{MM}{Matching Metric}
    \acro{MONAI}{Medical Open Network for Artificial Intelligence}
    \acro{MRI}{Magnetic Resonance Imaging}
    \acro{MS}{Matching Score}
    \acro{NETC}{Nonenhancing Tumor Core}
    \acro{NN}{Neural Network}
    \acro{NSD}{Normalized Surface Dice}
    \acro{PGT}{Peak Ground Truth}
    \acro{PQ}{Panoptic Quality}
    \acro{RQ}{Recognition Quality}
    \acro{RWMP}{Real World Model Performance}
    \acro{SQ}{Segmentation Quality}
    \acro{PanS}{Panoptic Segmentation}
    \acro{SNFH}{Surrounding Non-enhancing FLAIR Hyperintensity}
    \acro{SemS}{Semantic Segmentation}
    \acro{SQASSD}{Segmentation Quality Average Symmetric Surface Distance}
    \acro{t1c}{post-contrast T1-weighted}
    \acro{t1w}{pre-contrast T1-weighted}
    \acro{t2f}{T2-weighted Fluid Attenuated Inversion Recovery}
    \acro{FLAIR}{T2-weighted Fluid Attenuated Inversion Recovery}
    \acro{t2w}{T2-weighted}
    \acro{VerSe}{Large Scale Vertebrae Segmentation Challenge}

\end{acronym}


\newcommand{\eac}[1]{\textit{\ac{#1}}}
\newcommand{\eacp}[1]{\textit{\acp{#1}}}

\newcommand{\eacf}[1]{\textit{\acf{#1}}}
\newcommand{\eacfp}[1]{\textit{\acfp{#1}}}


\newcommand{\eacs}[1]{\textit{\acs{#1}}}
\newcommand{\eacsp}[1]{\textit{\acsp{#1}}}

\newcommand{\eacl}[1]{\textit{\acl{#1}}}
\newcommand{\eaclp}[1]{\textit{\aclp{#1}}}

==> flow/latex_evangelium.tex <==
\section{Latex evangelium}
\label{sec:evangelium}
% \label{sec:formatting}

Look at the .tex file to fully understand this \Cref{sec:evangelium}!


\subsection*{labels and referencing}
\begin{itemize}
    \item label sections that are supposed to be referenced with \label{sec:section_name}
    \item label figures with \label{fig:figure_name}
    \item label tables with \label{tab:table_name}
    \item label equations with \label{eq:equation_name}
    \item reference with \cref{sec:evangelium} or \Cref{sec:evangelium}
\end{itemize}

\subsection*{figures, tables and equations}
\begin{itemize}
    \item use a separate .tex file for each figure/table; this will make the final layout/typesetting process much smoother as we can easily move them around
    \item we put figures in a subfolder for each section called /fig
    \item use color-blind friendly palettes for example this \href{https://www.nature.com/articles/nmeth.1618}{one}
    \item observe the above label instructions
\end{itemize}

\subsection*{citations}
\begin{itemize}
    \item for citations we use \citep{kofler2021we} or \citet{kofler2021we}
\end{itemize}

\subsection*{acronyms}
\begin{itemize}
    \item define acronyms in /flow/acronyms.tex
    \item for singular acronyms use \eac{CNN} or \eacf{CNN}.
    \item for plural acronyms we use \eacp{CNN} or \eacfp{CNN}.
\end{itemize}

\subsection*{misc but important}
\begin{itemize}
    \item write in the present tense
    \item actively use spellcheckers such as Grammarly
    \item use auto code formatting and lining
    \item use one line of code for each sentence to enable proper version control with git
\end{itemize}


==> head/keywords.tex <==
\keywords{
    machine learning,
    deep learning,
    semantic segmentation,
    instance segmentation,
    NAKO,
    spine,
}

